High Throughput Data Center Topology Design

With high throughput networks acquiring a crucial role in supporting data-intensive applications, a variety of data center network topologies have been proposed to achieve high capacity at low cost. While this literature explores a large number of design points, even in the limited case of a network of identical switches, no proposal has been able to claim any notion of optimality. The case of heterogeneous networks, incorporating multiple line-speeds and port-counts as data centers grow over time, introduces even greater complexity. In this paper, we present the first non-trivial upper-bound on network throughput under uniform traffic patterns for any topology with identical switches. We then show that random graphs achieve throughput surprisingly close to this bound, within a few percent at the scale of a few thousand servers. Apart from demonstrating that homogeneous topology design may be reaching its limits, this result also motivates our use of random graphs as building blocks to explore the design of heterogeneous networks. Given a heterogeneous pool of network switches, through experiments and analysis, we explore how the distribution of servers across switches and the interconnection of switches affect network throughput. We apply these insights to a real-world heterogeneous data center topology, VL2, demonstrating as much as 43% higher throughput with the same equipment.

==> limitations_short.tex <==
\section{Limitations}
\label{sec:future}

While we have presented here foundational results on the design of both homogeneous and heterogeneous topologies, many interesting problems remain unresolved:

\begin{itemize}
\item We have not yet been able to obtain a non-trivial upper bound on the throughput of heterogeneous networks analogous to our result for homogeneous topologies. Such a bound would enable us to comment on how close to optimal our heterogeneous network designs are, and whether there is significant room for improvement.
\item While our analysis (\S\ref{subsec:analysis}) explains throughput behavior with respect to the interconnection of switches, we do not have a similar analysis for our result on server distribution (\S\ref{subsec:heterports}). Unfortunately, results that are simple to state are not always simple to prove.
\item Our results on heterogeneity only apply to networks with two types of switches. Generalizing these results to arbitrarily diverse networks would be valuable, but even just going from two classes of switches to three would cover a wider array of practical use cases.
\item Our work does not consider cable costs in its notion of optimality. While Jellyfish~\cite{jellyfish} showed that restricting cabling in the random graph to be similar to the fat-tree does not reduce the random graph's throughput by much, this still leaves open the possibility that some novel topology coupled with a novel cabling arrangement has much lower total cost.
\end{itemize}

%\paragraphb{Throughput bound for heterogeneous networks.} We have not yet been able to obtain a non-trivial upper bound on the throughput of heterogeneous networks analogous to our result for homogeneous topologies. 
%This requires a bound on average path length (rather than empirically measuring it, as in the upper bound of Fig.~\ref{fig:bounds:bound_hhbias}). 
%Such a bound would enable us to comment on how close to optimal our heterogeneous network designs are, and whether there is significant room for improvement.
%
%\paragraphb{Theoretical analysis of server distribution.} \ankitr{While our results in \S\ref{subsec:analysis} enable a sound understanding of throughput behavior with respect to the interconnection of switches, we did not show a similar analysis for our result on distributing servers across switches (\S\ref{subsec:heterports}). Unfortunately, results that are simple to state are not always simple to prove. \cut{Although the result is simple to state (\ie distribute servers in proportion to switch port count) and seems intuitive, a supporting analysis has so far eluded us.}}
%
%\paragraphb{Multiple switch types.} Our results on heterogeneity only apply to networks with two types of switches. Generalizing these results to arbitrarily diverse networks would be valuable, but even just going from two classes of switches to three would cover a wider array of practical use cases.
%%\cut{We conjecture that distributing servers in proportion to switch degrees is optimal for even more than two classes of switches.}
%
%\paragraphb{Formulaic optimal configuration prediction.} We do not yet have a formulaic way for predicting the best (random-graph based) topology for a given set of switches and servers. For the case of two classes of switches and uniform line-speed, we are able to build such topologies based on \emph{empirical} results. It is plausible however, that the methods we used to understand the behavior of throughput can be extended into a predictor of the best network configuration. This would allow us to design networks such as ones with multiple line-speeds without the need for simulation.
%
%\paragraphb{Co-optimization with cabling.} Our work does not consider cable costs in its notion of optimality. We do note that Jellyfish~\cite{jellyfish} showed that restricting cabling in the random graph to be similar to the fat-tree in complexity does not reduce the random graph's throughput by much. While this does imply that random graphs are superior to other topologies even in this setting, it is unknown whether they remain a close-to-optimal choice: perhaps an entirely different topology coupled with a novel cabling arrangement has much lower total cost while nearly preserving the throughput. 
%
%\paragraphb{A wider topology comparsion.} We have not so far produced a large-scale comparison of throughput of network topologies. Numerous topology designs for distributed hash tables~\cite{gummadi2003impact}, for example, tried to optimize for short paths, like our work.  However, they concentrated on topologies in which greedy routing found short paths, a constraint not relevant to data centers.  The topologies were intentionally homogeneous, and were not evaluated for throughput. \cite{swdc} applied a DHT-style small world topology to data centers, and was shown in \cite{jellyfish} to have lower throughput.  However, there are numerous other examples that could be evaluated.

